Multi-task Learning for Source Attribution and Field Reconstruction for Methane Monitoring

Inferring the source information of greenhouse gases, such as methane, from spatially sparse sensor observations is an essential element in mitigating climate change. While it is well understood that the complex behavior of the atmospheric dispersion of such pollutants is governed by the Advection-Diffusion equation, it is difficult to directly apply the governing equations to identify the source location and magnitude (inverse problem) because of the spatially sparse and noisy observations, i.e., the pollution concentration is known only at the sensor locations and sensors sensitivity is limited. Here, we develop a multi-task learning framework that can provide high-fidelity reconstruction of the concentration field and identify emission characteristics of the pollution sources such as their location, emission strength, etc. from sparse sensor observations. We demonstrate that our proposed framework is able to achieve accurate reconstruction of the methane concentrations from sparse sensor measurements as well as precisely pin-point the location and emission strength of these pollution sources.

==> research_goals.tex <==
% \section{Research Goals and Problem Setup}
% \subsection{Research Goals}
% We aim to jointly study the problem of predicting the complete spatio-temporal field of methane concentration from partial observations of a sparse sensor network in a 2D spatial-domain and solve the inverse problem of identifying  the location of pollution/emission sources and their emission characteristics (like emission strength, start time of emission, etc.) from these sensor measurements. We further assume that the concentration of the methane gas in the 2D domain is characterized by the Advection-Diffusion Equation, which can be leveraged to estimate the above quantities in a more robust manner.

% Therefore, the research goals in this paper can be summarized as follows:
% \begin{itemize}
%     \item Reconstruct the entire 2D Spatio-temporal field from the sparse sensor network observations.
%     \item Estimate the emission characteristics of the pollution/emission sources.
%     \item Obtain uncertainty estimates for each of the above predictions.
% \end{itemize} 

% \subsection{Formal Problem Setup}
% Let there be $N_s$ number of potential methane emission sources and $N_o$ number of sensors in the sensor network. We assume that the atmospheric diffusion is determined by the following Advection-Diffusion Equation:

% \begin{align}
% \label{eq:adv_diff_eqn}
%     \frac{\partial \phi}{\partial t}  + \mathbf{u} \nabla \phi - K \nabla^2 \phi = \sum_{i=1}^{N_s} q_i(\mathbf{x}, t); \:\: \mathbf{x} \in \mathbb{R}^2, t \in \mathbb{R}^+
% \end{align}

% where $\phi$ is the concentration of methane, $\mathbf{u}$ is the wind velocity field, $K$ is the turbulent diffusivity, and $q_i(x, t)$ is the emission strength of the $i-th$ emission source. The above partial differential equation (PDE) is defined in the 2D spatial domain $\mathbf{x} \in [a, b] \times [a, b]$ and time domain $t \in [0, T]$. Note that the above formulation of the Advection-Diffusion Equation assumes that the wind velocity field is divergence free, i.e., $\nabla u = 0$. 

% Let the time-series methane measurements of the $N_o$ sensors be $\Phi = \{\Phi_1, \Phi_2, ..., \Phi_{N_o}\}$, where $\Phi_{i}$ denotes the (time varying) sensor measurement of the $i$-th sensor, i.e., $\Phi_{i}=[\Phi_{i}^1, \Phi_{i}^2, ..., \Phi_{i}^{N_t}]$, and $N_t$ is the number of time steps. Also, the location of the $i$-th methane sensors are denoted by $\mathbf{x}_i^{\Phi}=(x_i^{\Phi}, y_i^{\Phi})$. Further note that the measurements $\Phi_i$ are observed at discrete uniform time intervals. The wind field $\mathbf{u} = [u_x, u_y]$ is known on a uniform 2D-grid in the spatial domain, i.e., $\mathbf{u} \in \mathbb{R}^{N_t \times N_x \times N_y \times 2}$, such that $N_x$ and $N_y$ are the number of discretizations of the input domain in $x$ and $y$ directions respectively. We further assume that our pollution sources are point sources, and can be realized as $q_{i}(x, t) = \delta(x-x_i^s, y-y_i^s).c_i$, where $c_i$ is the emission strength of the $i$-th emission source, $(x_i^s, y_i^s)$ is the location of the source, and $\delta$ is the dirac delta function. 

% Given the time series measurements of the sensor networks $\Phi \in \mathbb{R}^{N_o \times N_t}$, their locations $\mathbf{x}^{\Phi} = \{\mathbf{x}^{\Phi}_1, \mathbf{x}^{\Phi}_2, ..., \mathbf{x}^{\Phi}_{N_o}\}$, and the wind velocity field $\mathbf{u} \in \mathbb{R}^{N_t \times N_x \times N_y \times 2}$, the spatio-temporal field reconstruction problem can be formulated as estimating the methane concentration $\phi$ on the regular grid $N_t \times N_x \times N_y$. Additionally, we are also interested in estimating the emission characteristics of the $N_s$ potential emission sources, such as their constant emission strengths $\mathbf{c}=[c_1, c_2, ..., c_{N_s}]$, etc.



% % Problem Description,
% % General Problem setup and mathematical notations
% % (Original Problem setup. Divergence Free Condition)

% % Simplification of the problem to constant emitting sources.
% % Point sources (2d Gaussian Envelope): Why point sources would create problems for traditional PINN setup for inverse formulation?


% % Inverse problem setup: 
% % 1. From a single simulation (challenging)

% % 2.  Using AI to solve the inverse problem 

% % (requires multiple simulations)
% % How to generate so many simulations?
% % Physics-guided AI based Forward Model (F) - DeepONets / Fourier Neural Operators to generate fast simulations.
% % Generating the training data for the simplified problem (varying wind conditions and source strengths). Also, we need the initial condition to predict the concentration maps.

% % part 2: Given we know the exact PDE and the source locations with their respective strengths, fill in the missing data using the PDE. (Super-resolution type forward simulation), i.e., different initial condition. (somewhat along the line of the paper Levente shared)

% % % If part 2 can be done: we can compute the saliency maps ( dL/dq to update the q) by freezing the model weights.
% % % A small optimization is required to solve the inverse problem. (Probably not possible)

% % End to End training

% % Observations using Time AVERAGING





